Model order reduction of hyperbolic systems at the example of district heating networks

In this article a framework for the generation of a computationally fast surrogate model for district heating networks is presented. An appropriate model results in an index-1 hyperbolic, differential algebraic equation quadratic in state, exhibiting several hundred of outputs to be approximated. We show the existence of a global energy matrix which fulfills the Lyapunov inequality ensuring stability of the reduced model. By considering algebraic variables as parameters to the dynamical transport, the reduction of a linear, time varying (LTV) problem results. We present a scheme to efficiently combine linear reductions to a global surrogate model using a greedy strategy in the frequency domain. The numerical effectiveness of the scheme is demonstrated at different, existing, large scale networks.

==> amat.tex <==
\begin{align*}
A'=\left[
    \begin{array}{cccc|cccc|c|cccc}
      -q_1&&&&&&& a_{12}'&&&&&a_{1n}'\\
q_1&-q_1&&&&&&&&&&&\\
&\ddots&\ddots&&&&&&&&&&\\
&&q_1&-q_1&&&&&&&&&\\\hline
    &&&a_{21}'&     -q_2&&&&&&&&a_{2n}'\\
&&&&q_2&-q_2&&&&&&&\\
&&&&&\ddots&\ddots&&&&&&\\
&&&&&&q_2&-q_2&&&&&\\\hline
&&&&&&&&\ddots&&&&\\\hline
&&&a_{n1}'&&&&a_{n2}'&&      -q_n&&&\\
&&&&&&&&&q_n&-q_n&&\\
&&&&&&&&&&\ddots&\ddots&\\
&&&&&&&&&&&q_n&-q_n
  \end{array}
\right]\;.
\end{align*} 
(\hl{maybe replace by smaller figure})

==> questions.tex <==

\section{Check before submit}
Fig consistent and every figure is mentioned in the text
References correct and each is used
check spelling
core performance correct
resimulate runtimes
mention role of the decomposition and operator assembly
asympotic stability in more details

Really dont mention port Hamiltonian system?
Elsevier
Original research: control systems

Tables wie hochladen

Cover letter mandatory
https://service.elsevier.com/app/answers/detail/a_id/155/

Statement of contribution
Please include a short 'Author Statement'/'Statement of Contribution'//'Novelty Statement' with your submission.

A novelty statement is a brief statement describing the manuscript's potential impact and contribution to the field. Note this differs from an abstract, which describes what was done; the novelty statement needs to address why the research was undertaken (i.e., motivation and audience), the impact the research will have, and why it is a significant advance over past work done on the topic.

Declarations of interest: none. wo?

zip geht auch fuer Figures
pdf oder tex?

funding was wirklich relevant?
assign editor?

\section{Open questions}
\hl{Thanks to...Raul Borsche, Matthias Eimer? Or put them as author?}

asynchronous CFL ratios: ROM faster and with smaller error than full model
perfect transport:runtime scales worse
find a suitable ROM for a given error bound

\begin{itemize}
\item QBDAE? \cite{ahmad_moment-matching_2017}, \cite{benner_iterative_2017} 
\item mention Empirical gramians in the problem formulation section
\item why no DG tested?

\item main disadvantage of WENO: explicit in time scheme which requires a minimum number of order+1 cells on each pipeline, what further decreases the minimum number of steps. With non constant velocity its in addition first order anyway. Could be fixed by integrating over the polynomial expression in the velocity. Higher order is probably still better for non constant velocity since the timesteps in the explicit scheme are very small. \cite{borsche_high_2016}

\item Use  $\hat y$ for quantities in the frequency domain.
\item plot of modes of the system
\item at which reynolds are we operating?
\item order of the reduced scheme
\item development of full and reduced eigenvalues
\item flux combinations 
\item training phase for the reduction out of sample comparison
\item why high fidelity surrogate models really needed? Advantage for application?
\item IRKA works on the input output behaviour and can be connected to a global projection
\end{itemize}

Comparison to Balanced truncation running out the parameter range. DMD focusses on one timestep and a fixed time horizon. Out of sample comparison.
